YOLO for Knowledge Extraction from Vehicle Images: A Baseline Study

Accurate identification of vehicle attributes such as make, colour, and shape is critical for law enforcement and intelligence applications. This study evaluates the effectiveness of three state-of-the-art deep learning approaches YOLO-v11, YOLO-World, and YOLO-Classification on a real-world vehicle image dataset. This dataset was collected under challenging and unconstrained conditions by NSW Police Highway Patrol Vehicles. A multi-view inference (MVI) approach was deployed to enhance the performance of the models' predictions. To conduct the analyses, datasets with 100,000 plus images were created for each of the three metadata prediction tasks, specifically make, shape and colour. The models were tested on a separate dataset with 29,937 images belonging to 1809 number plates. Different sets of experiments have been investigated by varying the models sizes. A classification accuracy of 93.70%, 82.86%, 85.19%, and 94.86% was achieved with the best performing make, shape, colour, and colour-binary models respectively. It was concluded that there is a need to use MVI to get usable models within such complex real-world datasets. Our findings indicated that the object detection models YOLO-v11 and YOLO-World outperformed classification-only models in make and shape extraction. Moreover, smaller YOLO variants perform comparably to larger counterparts, offering substantial efficiency benefits for real-time predictions. This work provides a robust baseline for extracting vehicle metadata in real-world scenarios. Such models can be used in filtering and sorting user queries, minimising the time required to search large vehicle images datasets.

==> section_memory_time_notused.tex <==
\subsubsection{Time and Memory Analyses}


\begin{table}[h!]
\centering
\caption{Training Time and Memory Usage for YOLO  Classification Models}
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Training Time (hrs)}} & \multicolumn{3}{c}{\textbf{Memory Usage (GB)}} \\
& \textbf{Small} & \textbf{Large} & \textbf{X-Large} & \textbf{Small} & \textbf{Large} & \textbf{X-Large} \\
\hline
Colour         & 2.04  & 1.37  & 1.43  & 0.99  & 2.09  & 3.18 \\
Colour-TWO     & 21.39 & 7.32  & 26.78 & 1.01  & 2.00  & 3.47 \\
Make           & 1.83  & 1.61  & 2.87  & 0.93  & 2.07  & 3.33 \\
Shape          & 3.35  & 1.51  & 1.62  & 1.02  & 2.11  & 3.16 \\
\hline
\end{tabular}
\label{tab:memory-time}
\end{table}

\autoref{tab:memory-time}
The tables for  and TIME to train across YOLO-C, YOLOv11, and YOLO-W models provide a detailed comparison of resource requirements. For YOLO-C models, the memory requirements range from 0.93 GB for small models to 3.47 GB for x-large models. The time to train these models varies significantly, with the smallest models taking around 2.04 hours and the x-large models taking up to 26.78 hours, particularly for the colour-binary variant.

In the case of YOLOv11 models, the memory requirements are higher, with small models requiring around 9.03 GB and x-large models needing up to 35.30 GB. The time to train these models also increases with size, ranging from 3.10 hours for small models to 12.22 hours for x-large models. This indicates that YOLOv11 models, while potentially offering better performance, are more resource-intensive compared to Classification models.

\begin{table}[h!]
\centering
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Training Time (hrs)}} & \multicolumn{3}{c}{\textbf{Memory Usage (GB)}} \\
                                & \textbf{Small} & \textbf{Large} & \textbf{X-Large} & \textbf{Small} & \textbf{Large} & \textbf{X-Large} \\
\hline
Colour         & 3.10 & 6.79 & 9.27 & 9.03  & 22.63 & 17.75 \\
Colour-TWO     & 5.89 & 6.34 & 9.25 & 9.02  & 22.54 & 33.62 \\
Make           & 2.85 & 5.85 & 8.12 & 9.95  & 23.33 & 35.32 \\
Shape          & 8.93 & 6.32 & 12.22 & 8.97 & 22.53 & 29.12 \\
\hline
\end{tabular}
\caption{Training Time and Memory Usage for Different YOLOv11 Models}
\end{table}




YOLO-W models show a similar trend, with memory requirements ranging from 8.86 GB for small models to 26.1 GB for x-large models. The time to train these models varies from 3.92 hours for small models to 28.72 hours for large models, particularly for the colour-binary variant. Overall, these tables highlight the trade-offs between model size, memory requirements, and training time, providing valuable insights for optimising resource allocation based on 

\begin{table}[h!]
\centering
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Training Time (hrs)}} & \multicolumn{3}{c}{\textbf{Memory Usage (GB)}} \\
                                & \textbf{Small} & \textbf{Large} & \textbf{X-Large} & \textbf{Small} & \textbf{Large} & \textbf{X-Large} \\
\hline
Colour         & 3.92  & 7.19  & 9.30  & 8.86  & 20.80 & 26.10 \\
Colour-TWO     & 15.62 & 28.72 & 12.65 & 8.74  & 19.80 & 24.40 \\
Make           & 5.83  & 8.54  & 10.68 & 8.98  & 20.80 & 26.00 \\
Shape          & 5.51  & 6.64  & 8.68  & 8.92  & 21.00 & 26.00 \\
\hline
\end{tabular}
\caption{Training Time and Memory Usage for YOLO-World Models}
\end{table}
